Scaling Datalog for Machine Learning on Big Data

In this paper, we present the case for a declarative foundation for data-intensive machine learning systems. Instead of creating a new system for each specific flavor of machine learning task, or hardcoding new optimizations, we argue for the use of recursive queries to program a variety of machine learning systems. By taking this approach, database query optimization techniques can be utilized to identify effective execution plans, and the resulting runtime plans can be executed on a single unified data-parallel query processing engine. As a proof of concept, we consider two programming models--Pregel and Iterative Map-Reduce-Update---from the machine learning domain, and show how they can be captured in Datalog, tuned for a specific task, and then compiled into an optimized physical plan. Experiments performed on a large computing cluster with real data demonstrate that this declarative approach can provide very good performance while offering both increased generality and programming ease.

==> Makefile <==
TARGET=paper
TARGETTEX=${TARGET}.tex
TEXSRCS=paper.tex paper.bib source vldb.cls

all: ${TARGET}.pdf

${TARGET}.pdf: ${TEXSRCS} ${TARGET}.bbl
	( \
	pdflatex $(TARGET).tex; \
	while grep -q "Rerun to get cross-references right." $(<:.tex=.log); \
	do \
		pdflatex $(TARGET).tex; \
	done \
	)

${TARGET}.bbl: ${TARGET}.bib
	pdflatex ${TARGET}.tex
	bibtex ${TARGET}
	pdflatex ${TARGET}.tex

clean:
	rm -f \
	$(TARGETTEX:.tex=.aux) \
	$(TARGETTEX:.tex=.log) \
	$(TARGETTEX:.tex=.out) \
	$(TARGETTEX:.tex=.dvi) \
	$(TARGETTEX:.tex=.pdf) \
	$(TARGETTEX:.tex=.ps)


==> source/bgd-logic.tex <==

\begin{figure}
\begin{center}
\includegraphics[scale=0.4]{figures/bgd-logical-plan}
\caption{\label{fig:bgd-query-plan}Logical query plan for Iterative
  Map-Reduce-Update.}
\end{center}
\end{figure}

Figure~\ref{fig:bgd-query-plan} shows the logical query plan for
Iterative Map-Reduce-Update.  The plan is divided into two separate
data-flows, each labeled by the Datalog rules they implement in
Listing~\ref{lst:datalog-global}.  The dataflow labeled $G1$
initializes the global model using the \ol{init\_model} UDF\@, which
takes no input, and produces the initial model.

The $G2\mbox{--}3$ dataflow executes a single MapReduce round whenever
a new model is written.  The \ol{cross-product} operator combines the
model with each tuple in the training dataset, and then calls the
\ol{map} UDF on each result.  The mapped output is passed to a
\ol{group-all} operator, which uses the \ol{reduce} aggregate (e.g.,
sum) to produce a scalar value.  The aggregate value, together with
the model, is then passed to the \ol{update} UDF\@, the result of
which is checked for a new model.  If a new model is present then it
is written, which triggers a subsequent iteration.  Otherwise, the
\ol{update} output is dropped; terminating the execution.




==> source/hyracks-overview.tex <==
\label{subsec:hyracksruntime}
Hyracks~\cite{Borkar:2011ly} is a data-parallel runtime in the same general space as
Hadoop~\cite{hadoop} and Dryad~\cite{Isard:2007kx}. While Hadoop constrains computation
to ``map'' and ``reduce'' functions, Hyracks allows more flexible operators and forms of
data distribution. As compared to Hyracks, the Dryad system is a low-level dataflow
platform allowing unconstrained directed acyclic graphs representing arbitrary computation
with no special support for common patterns specific to data processing.

Hyracks accepts and manages data-parallel computations requested either by
direct end-users of Hyracks or by a compiler of a higher-level language.

\begin{figure}[h]
\centering
\includegraphics[scale=0.4, trim=0 675 0 0]{figures/tpch-jobspec}
\caption{Example Hyracks Job specification}\label{fig:example01_spec}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[scale=0.4, trim=0 700 0 0]{figures/tpch-han}
\caption{Example Hyracks Activity Node graph}\label{fig:example01_han}
\end{figure}

Jobs are submitted to Hyracks in the form of directed acyclic graphs that are made up of ``Operators'' and ``Connectors''.
To illustrate the key ideas in Hyracks via a familiar example,
Figure~\ref{fig:example01_spec} shows an example Hyracks job representing
a TPCH-like query that performs a join between a partitioned file containing
Customer records and another partitioned file containing Order records.
The result of the join is aggregated to count the popularities of orders by market
segment. Nodes in the figure represent Operators, and edges represent Connectors.
In Hyracks, Operators are responsible for consuming partitions of their inputs and
producing output partitions. Connectors perform redistribution of data between
different partitions of the same logical dataset.
For example, in Figure~\ref{fig:example01_spec}, the file scanners that scan the
Customer and Order files are each connected to the Join Operator by means of an M:N
Hash Partitioning Connector. This Connector ensures that all Customer (Order)
records reaching the Join Operator partitions agree on the hash-value of the
Customer's (Order's) CID attribute, thereby enabling each partition of the
Join Operator to peform a local join to produce output partitions.
In order to perform aggregation on the MKT\_SEGMENT attribute, the Join Operator's output
partitions are redistributed to the partitions of the GroupBy Operator using another
M:N Hash Partitioning Connector; this one hashes on the MKT\_SEGMENT attribute to ensure
that all records that match on the grouping attribute are directed to the same grouping
partition. Finally, the GroupBy Operator's output is written to a file by the FileWriter
Operator. The use of a 1:1 Connector between the GroupBy Operator and the FileWriter
Operator results in the creation of as many result partition files as GroupBy Operator
partitions.

Figure~\ref{fig:example01_han} illustrates the first step in the execution of the submitted Job by Hyracks. Operators in Hyracks are expanded into their constituent activities. For
example, the Join Operator in the example is made up of two activities, the Join Build Activity and the Join Probe Activity. This expansion is made possbile by APIs that Hyracks provides
to Operator implementors to enable them to describe such behavioral aspects of an operator.
As shown in Figure~\ref{fig:example01_han}, the Join Build Activity has a dashed edge
to the Join Probe Activity, which represents the blocking of the probe operation until
the build operation is complete. Although Hyracks does not understand the specifics of
the various activities of an operator, exposing the blocking characteristics of Operators
provides important scheduling information to the system. Also note that the GroupBy
Operator is similarly made up of two activities, which denotes the constraint that
it can produce no output until all of its input has been consumed.

\begin{figure} [h]
  \centering
  \includegraphics[scale=0.4, trim=0 500 0 0]{figures/tpch-rt}%{example01_rt}
  \caption{Parallel instantiation of the example}\label{fig:example01_rt}
  \label{fig:tpch-sizeup}
\end{figure}

Hyracks analyzes the Activity graph produced by the expansion described above to identify
the collections of Activities (Stages) that can be executed at any time (while adhering
to the blocking requirements of the Operators). Each Stage is parallelized and executed in
the order of dependencies. Figure~\ref{fig:example01_rt} shows the partitioned runtime graph
of the running example. The dashed polygons around the Operator Partitions represent the
stages that were inferred in the previous step of job execution. 

In addition to the Operator Implementor's API mentioned above,
Hyracks ships with a built-in set of standard ``database'' style operators such as
Filter, Hybrid-hash join, two flavors of Aggregators (Hash-based and Pre-sorted) and
a spilling Sort operator to name a few, that users can use to assemble dataflow jobs.
Hyracks also has a set of pre-implemented Connectors such as M-to-N Partitioning, Sort-Merging, and 1-to-1
Connectors. More details about Hyracks' computational model, as well as about its implementation and perormance,
are available in~\cite{Borkar:2011ly}.



==> source/logic-plan.tex <==

\begin{figure}
\begin{center}
\includegraphics[scale=0.4]{figures/query_plan_elements}
\caption{\label{fig:query-plan-elements}Elements of a logical query plan.}
\end{center}
\end{figure}


%These handcrafted plans use logical operators listed in Figure~\ref{fig:query-plan-elements}.
%We label each dataflow with the declarative rules they implement but omit the
%details of an exact compiler translation, which is future work.

In this section, we describe the logical query plans that implement the two
Datalog programs in Section~\ref{sec:declarative}.
Figure~\ref{fig:query-plan-elements} lists the elements that make up a logical
plan.  A dataset references a collection of tuple records.  We support the
usual suite of relational operators: cross-product, inner-join, projection,
selection, and group-by.  A line in the query plan connects operator outputs to
downstream operator inputs, with data flowing from left to right.  A line may
include a function name, which means that the function is applied to the tuple
values the flow through; similar to the {\bf foreach} operator in Pig Latin.


\subsection{Pregel Logical Plan}\label{sec:runtime_pregel}
\input{source/pregel-logic}

\subsection{Iterative Map-Reduce-Update Logical Plan}\label{sec:runtime_imr}
\input{source/bgd-logic}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> source/pregel-logic.tex <==

\begin{figure}
  \centering
    \includegraphics[scale=0.35]{figures/pregel_plan}
    \caption{\label{fig:pregel-logical-plan}Logical query plan for Pregel.}
\end{figure}


Figure~\ref{fig:pregel-logical-plan} shows the logical query plan for Pregel.
Each dataflow references rules from Listing~\ref{lst:datalog-local} they
implement.  The dataflows labeled $L1$ and $L2$ initialize the computation.  In
$L1$, we create the initial \ol{send} fact.  In $L2$, each tuple from the
training data is passed to the \ol{init\_vertex} UDF before being added to the
\ol{vertex} dataset.

The dataflow labeled $L3$-$L8$ iteratively executes supersteps in a bulk
synchronous processing model.  The \ol{send} dataset is first grouped by the
destination vertex identifier, and each such group of messages is aggregated by
the \ol{collect} UDF\@.  The \ol{vertex} dataset is also grouped by the vertex
identifier so that its most recent state can be selected by the \ol{max}
aggregate.  The two views form the \ol{collect} and \ol{local} IDB predicates,
which are joined along the vertex identifier attribute to produce the set of
vertices with outstanding messages.  The join result is passed to the
\ol{update} function to produce the \ol{superstep} view, which is subsequently
projected along two paths.  The top path projects the set of messages for the
next superstep onto the \ol{send} dataset.  The bottom path checks for a
non-null state object before projecting any resulting state objects onto the
\ol{vertex} dataset.



==> source/scalops.tex <==

ScalOps is a new high-level language for expressing workflows specific to
machine learning and graph analytics.  ScalOps directly supports iteration over
algorithms expressed as relational queries on the training and model data.  The
expressiveness of ScalOps follows from Chu et al.~\cite{Chu:2006fk}---showing
that many ML algorithms are naturally represented in relational algebra.
ScalOps goes beyond the prior work by (a)~capturing objective functions for
both local and global model types and (b)~automatically embedding those
objectives into recursive query plans that search the parameter space for
good models.

Like Pig, ScalOps combines the declarative style of SQL and the low-level
procedural style of MapReduce.  Like Spark, ScalOps can optimize its
runtime---the Hyracks parallel-database engine~\cite{Borkar:2011ly}---for
repeated access to data collections e.g., RDDs.  We differ from these previous
platforms in the following ways.
%
\begin{enumerate}
\item We provide an explicit looping construct that captures the 
  iteration in the runtime plan.
\item Since iteration is a first-class citizen in the language, we can
  automatically recognize the need to cache data.
\item Our runtime (Hyracks) is optimized for computations that span both
  in-memory and external memory datasets.
\item We directly support {\em cyclic} graphs of data-parallel
  operators (query plans).
\end{enumerate}
%
As such, ScalOps can efficiently handle a wider range of analytics
over any sized data in a scalable mannar.  The remainder of this
section describes ScalOps from a language perspective; what the
programmer writes.  We show examples of code for developing both
global and local model types.  Compilation of ScalOps code to an
executable form will be addressed in subsequent sections.  The primary
goal here is to show how ScalOps is able to capture objective
functions for both global and local models.

\subsection{Logistic Regression}\label{sec:scalops:clickpred}
%
\begin{lstlisting}[float, caption={Batch Gradient Descent in ScalOps}, label={fig:logreg}, language=scalops]
class Example(x:Vector, y:Double)

class State(w: VectorType, lastLoss:DoubleType, currentLoss:DoubleType){
  def converged = abs(currentLoss-lastLoss) < 1e-9
}

def lossAndGradient(w: Vector, ex: Example)={
  val loss = log(1 + exp(-exp.y * x.dot(w))
  val gradient = (-ex.y)/(1 + exp(ex.y * x.dot(w))
  return (loss, gradient)
}

def update(xy: Table[Example], s: State) = {
  val lg = xy.map(ex => lossAndGradient(s.w, ex))
  s.w -= lg.map(_._2).reduce(_+_)
  s.lastLoss = s.currentLoss
  s. currentLoss = lg.map(_._1).reduce(_+_)
}

def train(xy: Table[Example]) = {
  val s = State(zeros(1000), 0, 0)

  loop(s, !s.converged()) {s => update(xy, s)}
}
\end{lstlisting}
%
Logistic Regression is a popular classification technique. Given a
database of examples with binary labels, a global model is sought that
can predict the likelihood of a positive label for a yet unseen
example. Example applications include email spam classification and
click prediction for websites.  The data is represented as tuples
$(x,y)$, where $x \in R^n$ is a feature vector and $y \in [+1,-1]$ is
the label. \footnote{Note that the process of turning real world data
  into vectors --- feature extraction --- is well known to be
  expressible in a relational algebra and is therefore omitted in this
  example.}  Given a model vector $w \in R^n$, a prediction $f$ is
computed as $f = (1.0 + exp(-\inner{w}{x}))^{-1}$.  The training of a
logistic regression model thus amounts to finding the $w$ that best
corresponds to the data.\footnote{For the sake of presentation
  brevity, we omit the regularization needed for proper generalization
  performance of the model.}  As in the training of many global
machine learning models, this search is performed via convex
optimization, and one of the most common algorithm templates to do so
is batch gradient descent as seen in Listing~\ref{fig:logreg}:

The class~\ol{Example} represents an example with feature
vector~\ol{x} and label~\ol{y}.  The class~\ol{State} captures the
current state of the search: the model~\ol{w} with the last and
current loss value for convergence monitoring.  Note that the members
are of types with the suffix~\ol{Type}.  The operations on those types
extract an abstract syntax tree instead of actually performing them,
which is crucial for ScalOps' ability to extract the overall query
plan from otherwise imperative code.  A set of implicit conversions
allows the user to use the default scala types outside of the State
definition.  The method~\ol{converged} expresses the halting criterion
for the search.  The function~\ol{lossAndGradient} computes the
current loss --- a measure for how wrong the model is --- and the
gradient for an example. In \ol{update}, this function is applied to
all examples given to obtain the global gradient and loss. The global
gradient is used to update the model $w$, while the global loss is
stored for convergence monitoring.

In \ol{train} the final query plan is assembled. First, the \ol{State
  s} is initialized. Then, the iterative training is performed via
ScalOps' \ol{loop} construct, which accepts three parameters: (1) An
initial state of the search. (2) A function that determines whether
the loop shall continue or not based on the current state. (3) A
update function that accepts a state and returns a new one.



\subsection{PageRank}
\label{sec:scalops:pagerank}
\begin{lstlisting}[float, caption={PageRank in ScalOps},
  label={fig:pagerank}, language=scalops] 
class RState(rank :Float, iter :Int) extends State

class RMsg(src:Int, dst:Int, rank:Float) extends Message

class PageRank extends Vertex[RState, RMsg] {
  def initialize(page : Datum) = 
    RState(1 / TotalNumberOfVerticies(), 0) 

  def update(state: RState, msgs : Iterator[RMsg]) {
    var neighbors = 1.0
    var rank = state.rank
    if (state.iter > 0) {
      var sum = 0.
      for (msg <- msg) sum += msg.rank

      rank = 0.15 / msgs.size + 0.85 * sum
    }

    val outMsgs = ListBuffer[RMsg]
    for (msg <- msg)
    	outMsgs.append(
	  RMsg(MY_ID, msg.src, rank / neighbors))
    }

    val nextState = RState(rank, state.iter + 1)
    return (nextState, outMsgs)
  }

  def halt(state : RState) = state.iter < 30
}
\end{lstlisting}

In this section, we describe graph-based implementation of PageRank in
ScalOps.  The goal of PageRank is to compute a local model over the
web graph that identifies a rank for each vertex page.  This vertex
centric approach to implementing PageRank was first presented in
Pregel~\cite{pregel}.  We support an API similar to Pregel but differ
in how we map it to an underlying runtime.

Figure~\ref{fig:pagerank} replicates the PageRank algorithm from
Pregel~\cite{pregel} in ScalOps.  The \ol{PageRank} class extends
\ol{Vertex}, which is part of the ScalOps library.  Any \ol{Vertex}
class extension must implement three methods.  The \ol{initialize}
method accepts a \ol{Datum} object and returns a \ol{State} object,
which starts the computation.  The \ol{update} method accepts a
\ol{State} object and list of inbound \ol{Message} objects and returns
a new \ol{State} object and list of outbound \ol{Message} objects.
The \ol{update} method is called exactly once per superstep on each
active vertex.  The \ol{halt} method accepts a \ol{State} object and
returns a boolean value indicating its desire to remain active.  An
optional fourth method called \ol{sync} (not shown here) is
responsible for grouping inbound messages together prior to calling
\ol{update}.  It is similar to the combiner function made popular by
MapReduce and is also supported in Pregel.  The default \ol{sync}
method forms simple lists out of the inbound messages.


\subsection{Discussion}

ScalOps benefits from being a DSL internal to the Scala language,
primary in terms of programmer productivity and code readability, but
also in optimization opportunities.  In Scala, programmers have access
to all Java libraries and benefits of running on a JVM (ubiquity,
administrative tools, profiling, garbage collection, etc.).  ScalOps
seamlessly integrates into well-known IDEs (Eclipse, NetBeans, etc.)
thanks to the respective Scala IDE plugins.  ScalOps inherits a {\em
  static} type-checker from Scala; something foreign to Pig
programmers.  ScalOps uses Scala closures to package user code for
runtime execution.  In Pig, this code would be {\em external} Java
code that programmers would need to explicitly package into a Java
``jar'' file and ship to the runtime.  Moreover, Pig lacks visibility
into this code can not optimize based on associativity and
commutativity properties.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 

